Representation learning for improved interpretability and classification accuracy of clinical factors from EEG

Despite extensive standardization, diagnostic interviews for mental health disorders encompass substantial subjective judgment. Previous studies have demonstrated that EEG-based neural measures can function as reliable objective correlates of depression, or even predictors of depression and its course. However, their clinical utility has not been fully realized because of 1) the lack of automated ways to deal with the inherent noise associated with EEG data at scale, and 2) the lack of knowledge of which aspects of the EEG signal may be markers of a clinical disorder. Here we adapt an unsupervised pipeline from the recent deep representation learning literature to address these problems by 1) learning a disentangled representation using $\beta$-VAE to denoise the signal, and 2) extracting interpretable features associated with a sparse set of clinical labels using a Symbol-Concept Association Network (SCAN). We demonstrate that our method is able to outperform the canonical hand-engineered baseline classification method on a number of factors, including participant age and depression diagnosis. Furthermore, our method recovers a representation that can be used to automatically extract denoised Event Related Potentials (ERPs) from novel, single EEG trajectories, and supports fast supervised re-mapping to various clinical labels, allowing clinicians to re-use a single EEG representation regardless of updates to the standardized diagnostic system. Finally, single factors of the learned disentangled representations often correspond to meaningful markers of clinical factors, as automatically detected by SCAN, allowing for human interpretability and post-hoc expert analysis of the recommendations made by the model.

==> draft.tex <==
\section{Introduction}

This work applies a set of advances in unsupervised learning of disentangled representations to the problem of biomarker development from human electroencephalographic (EEG) data. $\beta$-variational autoencoders ($\beta$-VAE) are trained on resampled event-related potentials (ERPs)---neural timeseries (see Figure \ref{erp}), models with a high degree of disentanglement are identified, and a hybrid set of qualitative and quantitative assessment metrics are presented to examine the quality of the resulting models and the value of the technique for advancing SOTA analysis approaches for electrophysiology research in general.

\begin{figure}[htbp]
  \centering
  \includesvg{figs/erp}
  \caption{ERP---this is a placeholder waiting for our own image}
  \label{erp}
\end{figure}


\subsection{Background}

The foundational approach for defining and diagnosing mental health disorders has many well-identified limitations (CITES CITES). Under this framework, label reliability can be as low as $\alpha=.7$ between expert psychiatrists and psychologists---even with the benefit of a Structured Clinical Interview for DSM (SCID, Diagnostic and Statistical Manual of Mental Disorders) (CITES CITES). A challenge for this classification system is that it is symptom-based but uses polythetic criteria to define categories. This is problematic because many disorders do not have a fixed symptom profile; they present as a varying constellation of symptoms where any two people with the same SCID diagnosis can exhibit entirely different symptom expressions. For example, Major Depressive Disorder (MDD) has upwards of 1030 possible symptom combinations \citep{fried2015depression}. Compounding the problem, symptom-to-disease mapping is affected by co-morbidity. For example, the estimated anxiety and depression co-morbidity rate is XX\% (CITE). 

Such is the setting where machine learning-aided solutions would need to operate to contribute to solving the problem. The highest quality labels are collected from the SCID---where expert clinicians disagree upwards of 30\% of the time. The binary disease classification label must cover hundreds of idiosyncratic expressions within a single disorder.

This framing calls for an unsupervised approach. The inputs are noisy measures that only carry reliable signal in a subset of the positive cases; the science lacks consensus on the basic nature of the outputs. Thus, one learning objective that remains viable is to try to disentangle the statistical regularities of the input signal so that the learned representation can continue to be useful when the label taxonomy evolves. There are many benefits to an approach like this if broad regularities in disease and symptom expression can be objectively captured with unsupervised learning. At the least, an interpretable, factorized representation of these regularities has potential to advance understanding of the symptomology of the disease and the processing of ERPs in general.


%Whether these techniques are utilized for signal processing (e.g., ICA), or machine learning applications (e.g., CSP), they are calibrated using subject-specific training data. Such a requirement, however, reinforces the need for a large number of trials to reduce the likelihood of overfitting during the training process. Furthermore, these approaches make a number of assumptions about the data, such as non-Gaussianity, stationarity, whiteness, or statistically independent unitary dimensions, which may not extend to cross-session, cross-subject, or cross-experiment analyses. For example, ICA, CSP, and HDCA all utilize some form of spatial filtering, which can quickly become sub-optimal with slight variations in EEG electrode placement, as occurs across subjects or recording sessions (Marathe et al., 2016). ICA can converge on differing solutions for the same subject over different temporal epochs (Hsu et al., 2018) or fail to capture signal variance due to enforcement of statistical independence (Gordon et al., 2015). In short, we are not aware of any neural decoding approaches that can be robustly applied across datasets or experimental paradigms, such that they do not require subject-, or at least experiment-, specific training data.



\subsection{$\beta$-VAE for Unsupervised Disentangled Representation Learning}

\paragraph{Why seek disentanglement in biomarker representation learning?} The approach presented here is predicated on the idea that disentangled representations will be well-suited to solve a diverse set of EEG--psychopathology measurement problems. The utility of latent or factorized representations for EEG/ERP signal analysis is well-known, e.g., the use of Independent Components Analysis (ICA) and the regression-based rERP framework \citep{delorme2004eeglab, makeig2004mining, smith2015regression}. Our contribution is to test a representation learning technique that explicitly leverages the \textit{shared statistical strength} of generative modeling of the problem space, capturing the regularities of an objectively-measured biomarker with purely unsupervised learning \citep{bengio2013better}. 

The canonical ERP-as-biomarker processing problem involves de-noising EEG segments and analyzing particular \textit{components}---the stereotyped peaks and valleys of the waveform that reliably manifest in the post-stimulus presentation interval with around 100ms precision. Noise is prevalent on the x (time) and y (amplitude) axes of the waveform. A diverse set of psychological phenomena have been linked to these components. Unfortunately, component measurements are not independent: components can significantly overlap; later occurring components are affected by earlier components in the time series. Additionally, blinks and other eye and muscle movement (measured as the electrooculogram, EOG), nearby electronics and line noise, hardware quality, and electrode--scalp contact properties all distort the signal as well. Identifying these discrete sources of noise in the signal is usually the responsibility of lab technicians who watch nearly every epoch of EEG during data collection to maintain quality and then develop an offline processing pipeline where each EEG epoch is examined by trained staff. In terms of analysis, any discriminative model building will need target labels and must have an implicit (at the least) position on the issues presented above, i.e., the reliability of the existing mental health taxonomy.   

Therefore, a sensible goal is to focus on unsupervised representation learning---to attempt to disentangle all of these unique sources of variance in the signal and learn a model that has a higher probability of generalizing to a diverse set of tasks. The ideal outcome is the encoder and decoder remain intact and the architecture for inference can be simple and dynamic based on developments in the scientific taxonomy of mental health disorders. We developed a convolutional $\beta$-VAE architecture to test this conjecture within the domain of processing and analyzing EEG data.

\paragraph{Variational Autoencoders.} Autoencoders are an unsupervised generative representation learning tool with applications that span the range of the field: vision, audition, time series, biosignals, etc. The algorithm's recent success is thanks in part to recent adaptations such as the stochastic variational layer, e.g., VAE, \citep{kingma2013auto} and variations that promote the learning of disentangled representations, e.g., $\beta$-VAE, \citep{higgins2017beta}, MMD). Elaboration of relevance of \citep{higgins2017beta}

\paragraph{Unsupervised Disentanglement Ranking (UDR).} summary of \citet{duan2019unsupervised}, what it means here

\paragraph{Symbol-Concept Association Network (SCAN).} summary of \citet{higgins2017scan}, what it means here

\subsection{EEG as a Biomarker for Psychopathology.}

Electroencephalography (EEG) is the measurement of electrical current propagated from neuronal activity (and other sources) as measured at the scalp of humans and other animals. There are myriad potential applications for online EEG decoding but the promise of this technology to ``read the mind'' has yet to be realized. A critical motivating question for this work is how ANN-based solutions can continue to make progress in a domain where the stakes are life and death, the data are difficult to collect and label, and the brain processes that govern the signal are poorly understood? Reward; Arousal; REVIEW REVIEW CITE CITE. The use of matrix factorization techniques to facilitate EEG/ERP analysis is not novel \citep{smith2015regression} (CITE CITE how much due diligence needed here?).

\paragraph{LPP as a biomarker for anhedonia.} This work targets one of the two cardinal symptoms of MDD: Anhedonia is the the absence of arousal in the presence of arousing stimuli (CITE). One established approach for objectively quantifying this symptom is the use of EEG/ERP to measure neural responses elicited by arousing and non-arousing visual stimuli \cite{brown2012functional}. Research in this domain has uncovered a stereotyped neural activation pattern in healthy control participants where arousing stimuli evoke a Late Positive Potential (LPP) in ERPs---the averaged timeseries of stimulus-timelocked EEG recordings. This pattern has been identified as a potential biomarker for depression because (on average) this positive deflection in amplitude is attenuated or absent in individuals who exhibit symptom of anhedonia---i.e., these people do not experience arousal; they do not show the stereotyped LPP common in the ERPs of healthy controls.

\subsection{The Present Study}

\paragraph{Overview.} The goals of this work are to test a pipeline for learning disentangled representations on the hard problems of psychopathology biomarker development and experimental analysis of EEG/ERP data generally. People diagnosed with MDD often report symptoms of anhedonia, e.g, a loss of interest or pleasure; no positive feelings. An experimental paradigm designed to objectively measure the experience of this symptom with EEG was used to collect data from a sample of healthy control participants and people diagnosed with anxiety and depression (among other mental illnesses). $\beta$-VAE models were trained to represent and reconstruct single EEG segments and ERPs and evaluated to highlight the effectiveness of disentangled representations for the classification problem and the phenomenology of the EEG signal. 

\paragraph{Evaluation.} Models trained on single EEG segment--trajectories and averaged trajectories (ERPs) were evaluated with respect to a series of baselines that showcase the effectiveness of $\beta$-VAEs and disentangled representations. The ``baseline'' analysis technique is a faithful reproduction of the typical approach for basic research in clinical psychology. We compare this baseline to learned $\beta$-VAE representations coupled with logistic regression or SCAN.   

\paragraph{Impact.} What does success look like in this application? The ideal output of the disentanglement pipeline in this domain would be embedding models that have well-learned (1) the LPP delta effect, i.e., the critical condition difference elicited in the arousing visual evoked potential (VEP) experimental paradigm, (2) the stereotyped componentry of the ERP waveform, and (3) signal artifacts like muscle movement and the EOG. Such a model would reduce the dimensionality of the EEG signal to a more manageable size, it would reduce the burden of the decision to focus on particular time windows common to conventional analysis techniques. Concretely, we predict that high rankings in terms of disentanglement will correspond to increased classification accuracy on our assessment labels---demographics (e.g., age, gender), data collection characteristics (e.g,. collection site), and SCID-based diagnosis labels.   

Implications of success for the technique for psychopathology. Implications of success for the technique for electrophysiology. ML impact.

\section{Method}

$\beta$-VAEs were trained to represent and reconstruct ERPs collected in an emotional arousal paradigm with a sample of healthy control participants and individuals diagnosed with depression and anxiety disorders. The models were evaluated with contemporaneous and longitudinal symptom and diagnosis data. See supplemental materials repository We make available trained models; the training and evaluation datasets could not be released due to licensing but are possible to release on request.  

\subsection{Data}

\paragraph{Participants.} The data were collected as part of a multi-site mental health study. Participants ($N=758, age_{\bar{X}}=16.7, age_{range}=11.0-59.8$, 398 female) provided informed consent and then completed an array of EEG tasks, completed a SCID, and a number of other self-report measures of mental health. The models were trained with data collected from a visual evoked potential paradigm where positive and neutral stimuli from IAPS were presented while EEG was collected. 

\begin{table}[t]
%\vskip 0.1in
\begin{center}
\begin{scriptsize}
\begin{sc}
\begin{tabular}{ccccrr}
\toprule
            &       &   &     &     &\\
Site & AgeGroup & Gender & Diagnosis & Axis 1 & Depression     \\
\midrule
Site 1 & adult & F & 0.0 &   35 & 35\\ % FSU\_WAVE1
            &       &   & 1.0 &   59 & 59\\
            &       & M & 0.0 &   11 & 11\\
            &       &   & 1.0 &   12 & 12\\
Site 2 & child & F & 0.0 &   72 & 95 \\ % SDSU\_D2018
            &       &   & 1.0 &   31 & 8 \\
            &       & M & 0.0 &  101 & 119 \\
            &       &   & 1.0 &   19 & 1 \\
Site 3 & child & F & 0.0 &   82 & 128\\ % fsu\_d2018b50
            &       &   & 1.0 &   57 & 11\\
            &       & M & 0.0 &   98 & 150\\
            &       &   & 1.0 &   54 & 2\\
Site 4 & child & F & 0.0 &   41 & 58\\ % fsu\_d2018w8
            &       &   & 1.0 &   21 & 4\\
            &       & M & 0.0 &   45 & 63\\
            &       &   & 1.0 &   20 & 2\\
\bottomrule
\end{tabular}
\end{sc}
\caption{Participant label distribution}
\label{tbl_participant_demos}
\end{scriptsize}
\end{center}
% \vskip -0.2in
\end{table}

\paragraph{Stimuli and Experimental Design.} We operationalized arousal potential with the International Affective Picture System (IAPS) in an EEG/ERP collection paradigm proven to elicit the LPP (CITES). Participants were shown positive and neutrally-arousing images from IAPS while the signal was recorded with a Brain Vision Brain Amp DC amplifier.TODO: sample stims, more info

\paragraph{EEG Preprocessing.}

An automated preprocessing pipeline was developed that...Did ICA. The final step in the preprocessing pipeline was to exclude anomalous trials (EEG segments) from each participants data. In order of application, a raw maximum amplitude threshold was applied at \SI{\pm.005}{\volt}, the data were normalized per-participant to zero mean and unit variance and a standard deviation threshold was applied at $|\sigma|>=5$, finally standard deviation ``transients'' (i.e., deflections in the EEG time series between $t$ and $t+1$ where $|\sigma|>=3$) were identified and the associated trials were removed.  

\subsection{Model Architecture}

The VAE model used here is quite similar to the original architecture proposed by \citet{kingma2013auto} with the additional tuned hyperparamter, $\beta$ \citep{higgins2017beta}. The convolutional $\beta$-VAE was built to represent ERPs sampled from stimulus-time-locked segments of EEG timeseries from 3 channels (sensors). Critically, electrode site and experimental condition were presented to the model on the volume axis of the input without convolution. In other words, the activation of the latent encoding was affected by the information on each channel by condition combination, but these input streams were preserved, i.e., not convolved across channels or experimental condition. Thus each observation consisted of six, resampled EEG timeseries: 256 timepoints collected from \SI{-250}{\milli\second} to \SI{772}{\milli\second} (relative to stimulus presentation) sampled at 250hz for each electrode (Fz, Cz, Pz) by condition (neutral image, arousing image) combination. 

\subsection{Model Evaluation}

\paragraph{Baseline---logistic regression on LPP condition delta.} The canonical analysis approach for psychophysiology research with EEG is to meticulously collect data, hand-tune a preprocessing pipeline and then perform inferential statistics over regions of interest in the temporal and/or frequency domains. In studies on the LPP (and ERP componentry in general), the average amplitude difference between conditions is extracted for time windows of interest. The result is a timeseries of the amplitude difference between conditions, often used as the dependent measure for regression. We follow this process for the baseline comparison.    

% \paragragh{} The constraints presented above yield one guiding tenet for the evaluation of data representations in this research domain---maintain a generative, unsupervised learning curriculum for as long as possible to minimize the impact of low-reliability data (e.g., labels). Evaluation includes a typical analysis approach found in the EEG literature, a hybrid generative/discriminative assessment of learned representations from $\beta$-VAE, and an evaluation of the representations identified by this hybrid approach as compared to disentangled representations as discovered by UDR. 

\paragraph{Symbol--Concept Association Network evaluation.} SCAN was used to ...

\section{Results}

%\setlength{\tabcolsep}{2pt}
\begin{table}[t]
%\vskip 0.1in
\begin{center}
\begin{scriptsize}
\begin{sc}
\begin{tabular}{ll|cc|cc|cc|cc|cc}
\toprule
\multicolumn{2}{l|}{} & \multicolumn{2}{c|}{Age} & \multicolumn{2}{c|}{Gender} & \multicolumn{2}{c|}{Site} & \multicolumn{2}{c|}{Depression} & \multicolumn{2}{c}{Axis 1 } \\
& & ERP & SMPL & ERP & SMPL & ERP & SMPL & ERP & SMPL & ERP & SMPL \\
\midrule
\multicolumn{2}{l|}{Chance}         & \multicolumn{2}{c|}{0.50} &\multicolumn{2}{c|}{0.50} &\multicolumn{2}{c|}{0.25} &\multicolumn{2}{c|}{0.50} & \multicolumn{2}{c}{0.50} \\
\midrule
\multicolumn{2}{l|}{Baseline (ERP)}         & 0.74 & 0.56 & 0.52 & 0.51 & 0.38 & 0.30 & 0.64 & 0.56 & 0.52 & 0.52 \\
\multicolumn{2}{l|}{Baseline (SMPL)}         & 0.69 & 0.54 & 0.52 & 0.52 & 0.36 & 0.30 & 0.61 & 0.54  & 0.52 & 0.52 \\
\midrule
\multirow{2}{*}{SCAN (ERP)}  & Dis     & 0.78 & \textbf{0.64} & 0.58 & 0.50 & 0.39 & 0.30 & \textbf{0.68}  & \textbf{0.59}  & 0.54 & 0.52  \\
                       & Ent     & 0.48 & 0.50 &  0.48 & 0.50 & 0.21 & 0.25 & 0.50 & 0.49 & 0.50 & 0.50  \\

\multirow{2}{*}{SCAN (SMPL)} & Dis      & 0.73 & 0.59 & 0.57 & 0.53 & 0.38 & 0.30 & 0.67 & 0.56 & 0.55 & 0.50 \\
                            & Ent     & 0.41 & 0.45 & 0.43 & 0.46 & 0.16 & 0.20 & 0.46 & 0.49 & 0.53 & 0.49 \\


\midrule                            
\multirow{2}{*}{Classifier (ERP)} & Dis     & \textbf{0.85} & 0.62  & 0.66 & 0.53 & \textbf{0.51} & 0.34 & \textbf{0.68} & \textbf{0.59} & \textbf{0.60} & \textbf{0.55}  \\
                            & Ent     & \textbf{0.85} &  0.62 & \textbf{0.68} & \textbf{0.57} & 0.48 & \textbf{0.37} & \textbf{0.69} & \textbf{0.59} &  \textbf{0.60} & \textbf{0.56} \\

\multirow{2}{*}{Classifier (SMPL)} & Dis    & 0.76 & \textbf{0.65}  & 0.58 & 0.53 &  0.40  & \textbf{0.36}  & 0.67 & \textbf{0.58}  & 0.56 & \textbf{0.56} \\
                            & Ent      & 0.76 & \textbf{0.65} & 0.63 & \textbf{0.57} & 0.46 & \textbf{0.36} & 0.66 & \textbf{0.58}  & \textbf{0.59} & 0.54 \\                                   
\bottomrule
\end{tabular}
\end{sc}
\caption{Balanced classification accuracy results for predicting various factors from EEG signals. ERP - averaged trajectories, SMPL - single sampled EEG trajectories. Balanced classification calculated as the average of precision and recall. Baseline - logistic regression trained from late positive potential (400-700~ms post stimulus onset) delta (pleasant-neutral) from each sensor (Fz, Cz, Pz), extracted either from ERPs or from single sample EEG trajectories. SCAN and Classifier refer to SCAN or logistic regression trained on top of either a disentangled (Dis) or entangled (Ent) $\beta$-VAE representations. When trained on the ERP inputs, all models are tested on either the same training ERPs or randomly sampled single EEG trajectory inputs. When trained on single EEG trajectories, all models are tested on either ERPs or randomly sampled single EEG trajectories that are different from the training ones. Both entangled and disentangled $\beta$-VAE representations result in classification accuracy improvements over the baseline. Training a classifier on top of $\beta$-VAE representations is generally better than training SCAN, but SCAN produces interpretable results (see Fig.~\ref{fig_traversals}. SCAN only works with disentangled $\beta$-VAEs. $\beta$-VAEs trained on single samples produce slightly lower accuracy than those trained on ERPs, but still outperform the baseline (including ERP training condition), suggesting that $\beta$-VAE representation learning increases accuracy while reducing the amount of training data by around 25x.}
\label{tbl_classification_results}
\end{scriptsize}
\end{center}
% \vskip -0.2in
\end{table}

%\setlength{\tabcolsep}{2pt}
\begin{table}[t]
%\vskip 0.1in
\begin{center}
\begin{footnotesize}
\begin{sc}
\begin{tabular}{cc|cc|cc|cc|cc}
\toprule
\multicolumn{2}{c|}{Age} & \multicolumn{2}{c|}{Gender} & \multicolumn{2}{c|}{Site} & \multicolumn{2}{c|}{Depression} & \multicolumn{2}{c}{Axis 1 } \\
Corr  & \textit{p} & Corr & \textit{p} & Corr & \textit{p} & Corr & \textit{p} & Corr & \textit{p} \\
\midrule
 0.28 & .01 & -0.1 & .31 & 0.19 & .06 & 0.33 & <.001 & 0.31 & <.001 \\
\bottomrule
\end{tabular}
\end{sc}
\caption{Correlation between disentanglement quality (as approximated by UDR score) of trained $\beta$-VAE models (n=100) and the resulting SCAN balanced classification accuracy for various factors. For age, depression and axis 1 higher disentanglement quality tends to result in higher SCAN classification accuracy.}
\label{tbl_correlation_results}
\end{footnotesize}
\end{center}
% \vskip -0.2in
\end{table}


\begin{figure}[htbp]
  \centering
  %\includesvg[width=1.\textwidth]{figs/sample_reconstructions_hor.svg}
  \includegraphics[width=1.\textwidth]{figs/sample_reconstructions_hor.png}
  \caption{Reconstructions (middle six columns) by three pre-trained $\beta$-VAE models (referred to as ``disentangled'', ``entangled'' and ``sample'') of single EEG trajectories (samples inputs) or their corresponding ERPs (ERP inputs). Each trajectory was obtained from a different participant. ``Disentangled'' and ``entangled'' models were pre-trained on the ERPs, while the ``sample'' model was pre-trained on single EEG trajectory samples (disentanglement did not affect the reconstruction performance of the models as tested in this plot, so a representation example is shown). Models pre-trained on ERPs are able to reconstruct ERP-like trajectories even from single EEG samples as presented, as demonstrated by the closer similarity of the ``disentangled'' and ``entangled'' reconstructions to ERP inputs vs Sample inputs regardless of the input condition. }
  \label{fig_sample_reconstructions}
\end{figure}


\begin{figure}[htbp]
  \centering
  %\includesvg[width=1.\textwidth]{figs/traversals_samples.svg}
  \includegraphics[width=1.\textwidth]{figs/traversals_samples.pdf}
  \caption{\textbf{A}: Latent traversals of a pre-trained disentangled $\beta$-VAE. Each rows reconstructs an ERP trajectory after varying the value of each latent dimension between [-2, 2] while keeping all other latents fixed to their inferred values. \textbf{B}: Inferred distributions for each of the 10 latent dimensions when symbols corresponding to different conditions of a single factor are presented to a SCAN pre-trained with the same $\beta$-VAE as in A. It is clear that different factors have become associated with different (often single) latent dimensions. For example, Axis 1 is represented by dimension z9. The presence (red) or absence (blue) of condition associated with Axis 1 is represented by the different narrow inferred Gaussian distributions centered around different opposite values of the respective latent. All other latent dimensions are reduced to the prior (unit Gaussian). \textbf{C}: five samples from each of the two conditions associated with the depression factor from the SCAN shown in B. Green - pleasant responses, blue - neutral responses from each sensor (Fz, Cz, Pz) (TODO check that this is correct!!). SCAN has learnt that the presence of depression is associated with a clear separation between responses in the two conditions. }
  \label{fig_traversals}
\end{figure}

\paragraph{Baseline}

As stated, we conducted an idiomatic approach for ERP analysis of the LPP effect to establish a baseline for the subsequent $\beta$-VAE representation assessment. In this approach, the amplitude delta between waveforms evoked from arousing and non-arousing stimuli is calculated and NHST is used to determine if the difference in LPP between healthy controls and people diagnosed with MDD is generalizable.        


% \begin{figure}
% \centering
% \includegraphics[scale=.25]{figs/PH_condelta_activation_factors_spearman.png}
% \caption{Placeholder fig for $\beta$-VAE latent activation by contemporaneous motivation factor correspondence. The null hypothesis is representable as the identity function. Latent activations patterns are more strongly related to the participant self report data in as much as the $p$-value lines bend toward the lower right quadrant of the plot.} 
% \end{figure}

\subsection{Latent Traversal}

\subsection{Effectiveness of SCAN}

\section{General Discussion}

How do we determine if the latent factorization has actually encoded something about the disease?

\subsection{Label Quality and the Definition of Depression}

What should the key takeaways be from the results, particularly with respect to the difficulty of the biomarker development problem for depression?

\subsection{Advances for electrophysiology research and applications}

The architecture used here was designed with a laser-focus on embedding the important between-condition differences that have been reliably found with NHST-based experimental paradigms. This was not a bottom-up approach to the problem, though there are dynamics in the temporal and frequency domains that could be contributing to the overall effectiveness of the approach (e.g., CITE ppathology + entropy work). Given the difficulty in extracting signal from one of the most reproducible biomarkers from the scientific study of MDD, our advice for future efforts is to always start with a top-down inquiry directed at known, reproducible phenomenon. It is a bonus if it turns out that models are utilizing unexpected variance in the signal but these outcomes must face the utmost level of scrutiny if broad conclusions about the phenomenology of the disease are made. HERE'S WHERE WE SAY SOMETHING WE THINK WE LEARNED ABOUT HUMANS THAT IS OBSERVABLE FROM THE RESULTS.  

\subsection{Value of controlling a Biomarker study end-to-end}

Many studies at the intersection of machine learning and medical neuroimaging rely on open datasets and accurate preprocessing on the part of the research teams or agencies that collect the data. Several advantages come from author involvement at every stage of this process. We would not have the insight we have here if the team was not multidisciplinary and integrally involved in the design of the studies for which the data was collect. Chief among these advantages is that the results and limitations of the data are well-situated---a naive take on these data and results might be that performance was not impressive. yada yada

\subsection{Conclusion}

This paper presented an unsupervised, generative representation learning technique designed to discover models with a high degree of disentanglement. The technique was deployed on a complex real world problem---measurement of EEG-based biomarkers for the diagnosis of mental health conditions---where the inputs and targets exhibit a high degree of noise and there is broad disagreement among humans about basic aspects of the problem setup. We compared disentangled $\beta$-VAEs to a frequentist analysis technique, entangled models AND ... The results show that this disentanglement pipeline can be an effective technique for learning a model of the target domain that is completely naive to the taxonomy of labels that humans expect to find in the data. This work provides the first evidence that disentanglement-focused representation learning and the resulting models are powerful measurement tools with immediately applicability to applied and basic research for clinical psychology and electrophysiology.  

% \section{Submission of conference papers to ICLR 2021}

% ICLR requires electronic submissions, processed by
% \url{https://openreview.net/}. See ICLR's website for more instructions.

% If your paper is ultimately accepted, the statement {\tt
%   {\textbackslash}iclrfinalcopy} should be inserted to adjust the
% format to the camera ready requirements.

% The format for the submissions is a variant of the NeurIPS format.
% Please read carefully the instructions below, and follow them
% faithfully.

% \subsection{Style}

% Papers to be submitted to ICLR 2021 must be prepared according to the
% instructions presented here.

% %% Please note that we have introduced automatic line number generation
% %% into the style file for \LaTeXe. This is to help reviewers
% %% refer to specific lines of the paper when they make their comments. Please do
% %% NOT refer to these line numbers in your paper as they will be removed from the
% %% style file for the final version of accepted papers.

% Authors are required to use the ICLR \LaTeX{} style files obtainable at the
% ICLR website. Please make sure you use the current files and
% not previous versions. Tweaking the style files may be grounds for rejection.

% \subsection{Retrieval of style files}

% The style files for ICLR and other conference information are available online at:
% \begin{center}
%   \url{http://www.iclr.cc/}
% \end{center}
% The file \verb+iclr2021_conference.pdf+ contains these
% instructions and illustrates the
% various formatting requirements your ICLR paper must satisfy.
% Submissions must be made using \LaTeX{} and the style files
% \verb+iclr2021_conference.sty+ and \verb+iclr2021_conference.bst+ (to be used with \LaTeX{}2e). The file
% \verb+iclr2021_conference.tex+ may be used as a ``shell'' for writing your paper. All you
% have to do is replace the author, title, abstract, and text of the paper with
% your own.

% The formatting instructions contained in these style files are summarized in
% sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

% \section{General formatting instructions}
% \label{gen_inst}

% The text must be confined within a rectangle 5.5~inches (33~picas) wide and
% 9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
% Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
% preferred typeface throughout. Paragraphs are separated by 1/2~line space,
% with no indentation.

% Paper title is 17~point, in small caps and left-aligned.
% All pages should start at 1~inch (6~picas) from the top of the page.

% Authors' names are
% set in boldface, and each name is placed above its corresponding
% address. The lead author's name is to be listed first, and
% the co-authors' names are set to follow. Authors sharing the
% same address can be on the same line.

% Please pay special attention to the instructions in section \ref{others}
% regarding figures, tables, acknowledgments, and references.


% There will be a strict upper limit of 8 pages for the main text of the initial submission, with unlimited additional pages for citations. Note that the upper page limit differs from last year!Authors may use as many pages of appendices (after the bibliography) as they wish, but reviewers are not required to read these. During the rebuttal phase and for the camera ready version, authors are allowed one additional page for the main text, for a strict upper limit of 9 pages.

% \section{Headings: first level}
% \label{headings}

% First level headings are in small caps,
% flush left and in point size 12. One line space before the first level
% heading and 1/2~line space after the first level heading.

% \subsection{Headings: second level}

% Second level headings are in small caps,
% flush left and in point size 10. One line space before the second level
% heading and 1/2~line space after the second level heading.

% \subsubsection{Headings: third level}

% Third level headings are in small caps,
% flush left and in point size 10. One line space before the third level
% heading and 1/2~line space after the third level heading.

% \section{Citations, figures, tables, references}
% \label{others}

% These instructions apply to everyone, regardless of the formatter being used.

% \subsection{Citations within the text}

% Citations within the text should be based on the \texttt{natbib} package
% and include the authors' last names and year (with the ``et~al.'' construct
% for more than two authors). When the authors or the publication are
% included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
% in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
% should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
% towards AI~\citep{Bengio+chapter2007}.'').

% The corresponding references are to be listed in alphabetical order of
% authors, in the \textsc{References} section. As to the format of the
% references themselves, any style is acceptable as long as it is used
% consistently.

% \subsection{Footnotes}

% Indicate footnotes with a number\footnote{Sample of the first footnote} in the
% text. Place the footnotes at the bottom of the page on which they appear.
% Precede the footnote with a horizontal rule of 2~inches
% (12~picas).\footnote{Sample of the second footnote}

% \subsection{Figures}

% All artwork must be neat, clean, and legible. Lines should be dark
% enough for purposes of reproduction; art work should not be
% hand-drawn. The figure number and caption always appear after the
% figure. Place one line space before the figure caption, and one line
% space after the figure. The figure caption is lower case (except for
% first word and proper nouns); figures are numbered consecutively.

% Make sure the figure caption does not get separated from the figure.
% Leave sufficient space to avoid splitting the figure and figure caption.

% You may use color figures.
% However, it is best for the
% figure captions and the paper body to make sense if the paper is printed
% either in black/white or in color.
% \begin{figure}[h]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
% \end{center}
% \caption{Sample figure caption.}
% \end{figure}

% \subsection{Tables}

% All tables must be centered, neat, clean and legible. Do not use hand-drawn
% tables. The table number and title always appear before the table. See
% Table~\ref{sample-table}.

% Place one line space before the table title, one line space after the table
% title, and one line space after the table. The table title must be lower case
% (except for first word and proper nouns); tables are numbered consecutively.

% \begin{table}[t]
% \caption{Sample table title}
% \label{sample-table}
% \begin{center}
% \begin{tabular}{ll}
% \multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
% \\ \hline \\
% Dendrite         &Input terminal \\
% Axon             &Output terminal \\
% Soma             &Cell body (contains cell nucleus) \\
% \end{tabular}
% \end{center}
% \end{table}

% \section{Default Notation}

% In an attempt to encourage standardized notation, we have included the
% notation file from the textbook, \textit{Deep Learning}
% \cite{goodfellow2016deep} available at
% \url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
% is not required and can be disabled by commenting out
% \texttt{math\_commands.tex}.


% \centerline{\bf Numbers and Arrays}
% \bgroup
% \def\arraystretch{1.5}
% \begin{tabular}{p{1in}p{3.25in}}
% $\displaystyle a$ & A scalar (integer or real)\\
% $\displaystyle \va$ & A vector\\
% $\displaystyle \mA$ & A matrix\\
% $\displaystyle \tA$ & A tensor\\
% $\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
% $\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
% $\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
% $\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
% $\displaystyle \ra$ & A scalar random variable\\
% $\displaystyle \rva$ & A vector-valued random variable\\
% $\displaystyle \rmA$ & A matrix-valued random variable\\
% \end{tabular}
% \egroup
% \vspace{0.25cm}

% \centerline{\bf Sets and Graphs}
% \bgroup
% \def\arraystretch{1.5}

% \begin{tabular}{p{1.25in}p{3.25in}}
% $\displaystyle \sA$ & A set\\
% $\displaystyle \R$ & The set of real numbers \\
% $\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
% $\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
% $\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
% $\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
% $\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
% $\displaystyle \gG$ & A graph\\
% $\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
% \end{tabular}
% \vspace{0.25cm}


% \centerline{\bf Indexing}
% \bgroup
% \def\arraystretch{1.5}

% \begin{tabular}{p{1.25in}p{3.25in}}
% $\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
% $\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
% $\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
% $\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
% $\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
% $\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
% $\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
% $\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
% \end{tabular}
% \egroup
% \vspace{0.25cm}


% \centerline{\bf Calculus}
% \bgroup
% \def\arraystretch{1.5}
% \begin{tabular}{p{1.25in}p{3.25in}}
% % NOTE: the [2ex] on the next line adds extra height to that row of the table.
% % Without that command, the fraction on the first line is too tall and collides
% % with the fraction on the second line.
% $\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
% $\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
% $\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
% $\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
% $\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
% $\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
% $\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
% $\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
% $\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
% \end{tabular}
% \egroup
% \vspace{0.25cm}

% \centerline{\bf Probability and Information Theory}
% \bgroup
% \def\arraystretch{1.5}
% \begin{tabular}{p{1.25in}p{3.25in}}
% $\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
% $\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
% a variable whose type has not been specified\\
% $\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
% $\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
% $\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
% $\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
% $\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
% $\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
% $\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
% over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
% \end{tabular}
% \egroup
% \vspace{0.25cm}

% \centerline{\bf Functions}
% \bgroup
% \def\arraystretch{1.5}
% \begin{tabular}{p{1.25in}p{3.25in}}
% $\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
% $\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
%   $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
%   (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
% $\displaystyle \log x$ & Natural logarithm of $x$ \\
% $\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
% $\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
% $\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
% $\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
% $\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
% $\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
% \end{tabular}
% \egroup
% \vspace{0.25cm}



% \section{Final instructions}
% Do not change any aspects of the formatting parameters in the style files.
% In particular, do not modify the width or length of the rectangle the text
% should fit into, and do not change font sizes (except perhaps in the
% \textsc{References} section; see below). Please note that pages should be
% numbered.

% \section{Preparing PostScript or PDF files}

% Please prepare PostScript or PDF files with paper size ``US Letter'', and
% not, for example, ``A4''. The -t
% letter option on dvips will produce US Letter files.

% Consider directly generating PDF files using \verb+pdflatex+
% (especially if you are a MiKTeX user).
% PDF figures must be substituted for EPS figures, however.

% Otherwise, please generate your PostScript and PDF files with the following commands:
% \begin{verbatim}
% dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
% ps2pdf mypaper.ps mypaper.pdf
% \end{verbatim}

% \subsection{Margins in LaTeX}

% Most of the margin problems come from figures positioned by hand using
% \verb+\special+ or other commands. We suggest using the command
% \verb+\includegraphics+
% from the graphicx package. Always specify the figure width as a multiple of
% the line width as in the example below using .eps graphics
% \begin{verbatim}
%   \usepackage[dvips]{graphicx} ...
%   \includegraphics[width=0.8\linewidth]{myfile.eps}
% \end{verbatim}
% or % Apr 2009 addition
% \begin{verbatim}
%   \usepackage[pdftex]{graphicx} ...
%   \includegraphics[width=0.8\linewidth]{myfile.pdf}
% \end{verbatim}
% for .pdf graphics.
% See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

% A number of width problems arise when LaTeX cannot properly hyphenate a
% line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

==> related_work.tex <==
\section{Related work}
The typical EEG classification pipeline consists of a pre-processing stage, during which the signal is averaged, denoised, and cleaned of interfering artifacts, like the blink response. This is usually done through the use of Independent Components Analysis (ICA) and the regression-based rERP framework \citep{delorme2004eeglab, makeig2004mining, smith2015regression, jung2000removing}. The result is in an ERP with pronounced components. The researcher then extracts the components relevant to the classification objective and uses Support Vector Machines (SVM), Linear Discriminant Analysis (LDA), Random Forest (RF) or regularised Logistic Regression (LR) to obtain the final classification results \citep{parvar2015detection, guler2007multiclass, subasi2010eeg, tomioka2007logistic, bashivan2016learning}. Recent advances in deep learning have prompted research into end-to-end classification using convolutional and/or recurrent neural networks \citep{bashivan2016learning, mirowski2009classification, cecotti2011convolutional, guler2005recurrent, wang2018convolutional, farahat2019convolutional, solon2019decoding, cecotti2014single} with minimal EEG signal pre-processing through a combination of older tools, like ICA, and basic representation learning using Restricted Boltzman Machines (RBMs) \citep{plis2014deep}. The problem with applying end-to-end classification using deep neural networks (DNNs), however, is that DNNs operate best in the big data regime with clean, well-balanced ground truth labels. In contrast, even the larger of available EEG datasets typically contain only a few hundred datapoints. The problem is compounded by noisy and unbalanced classification labels, with the majority of data coming from healthy controls.  As far as we are aware, no one has successfully applied modern representation learning techniques to the problem of identifying clinical biomarkers in the EEG data before.

